A Piece of My Mind: A Sentiment Analysis Approach for Online Dispute Detection

We investigate the novel task of online dispute detection and propose a sentiment analysis solution to the problem: we aim to identify the sequence of sentence-level sentiments expressed during a discussion and to use them as features in a classifier that predicts the DISPUTE/NON-DISPUTE label for the discussion as a whole. We evaluate dispute detection approaches on a newly created corpus of Wikipedia Talk page disputes and find that classifiers that rely on our sentiment tagging features outperform those that do not. The best model achieves a very promising F1 score of 0.78 and an accuracy of 0.80.

==> lexicon.tex <==
\begin{table*}[ht]
\centering
    {\fontsize{8}{9}\selectfont
    \begin{tabular}{|p{160mm}|}
    \hline
	\textsc{Positive}\\ \hline
	please elaborate, nod, await response, from experiences, anti-war, profits, promises of, is undisputed, royalty, sunlight, conclusively, badges, prophecies, in vivo, tesla, pioneer, published material, from god, plea for, lend itself, geek, intuition, morning, anti \texttt{SentiWord}$_{neg}$, connected closely, Rel(undertake, to), intelligibility, Rel(articles, detailed), of noting, for brevity, Rel(believer, am), endorsements, testable, source carefully\\ \hline
	\textsc{Negative} \\ \hline
	: (, TOT, ?!!, in contrast, ought to, whatever, Rel(nothing, you), anyway, Rel(crap, your), by facts, purporting, disproven, Rel(judgement, our), Rel(demonstrating, you), opt for, subdue to, disinformation, tornado, heroin, Rel(newbies, the), Rel (intentional, is), pretext, watergate, folly, perjury, Rel(lock, article), contrast with, poke to, censoring information, partisanship, insurrection, bigot, Rel(informative, less), clowns, Rel(feeling, mixed), never-ending\\ \hline
	\end{tabular}
	}
	\vspace{-4mm}
    \caption{\small Example terms and relations from our online discussion lexicon. We choose for display terms that do not contain any seed word.}
    \label{tab:lexicon_example}
\end{table*}


So far as we know, there is no lexicon available for online discussions. Thus, we create from a large-scale corpus via \textit{label propagation}.
%\subsection{Label Propagation Algorithm}
The label propagation algorithm, proposed by~\newcite{citeulike:310457}, is a semi-supervised learning method. In general, it takes as input a set of seed samples (e.g. sentiment words in our case), and the similarity between pairwise samples, then iteratively assigns values to the unlabeled samples (see Algorithm~\ref{alg:label_prop}).
%We describe the lexicon induction process in Algorithm~\ref{alg:label_prop}. 
The construction of graph $G$ is discussed in Section~\ref{subsec:graph}. %This algorithm has been shown to produce comparable performance to state-of-the-art systems that use a sophisticated optimization framework~\cite{conf/acl/FengKKC13}. 
Sample sentiment words in the new lexicon are listed in Table~\ref{tab:lexicon_example}.

\begin{algorithm}
\begin{small}
\footnotesize
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{$G=(V,E), w_{ij}\in [0, 1]$, positive seed words $P$, negative seed words $N$, number of iterations $T$}
\Output{\{$y_{i}$\}$_{i=0}^{\mid V \mid-1}$}
\BlankLine
$y_{i}=1.0$, $\forall v_{i}\in P$\\
$y_{i}=-1.0$, $\forall v_{i}\in N$\\
$y_{i}=0.0$, $\forall v_{i} \notin P\cup N$\\
\BlankLine

\For{$t=1 \cdots T$}{
	$y_{i}=\frac{\sum_{(v_{i}, v_{j})\in E} w_{ij} \times y_{j}}{\sum_{(v_{i}, v_{j})\in E} w_{ij}}$, $\forall v_{i}\in V$\\
	$y_{i}=1.0$, $\forall v_{i}\in P$\\
	$y_{i}=-1.0$, $\forall v_{i}\in N$\\
}

\end{small}
\vspace{-1mm}
\caption{\small The label propagation algorithm~\cite{citeulike:310457} used for constructing online discussion lexicon.}
\label{alg:label_prop}
\end{algorithm}

\subsection{Graph Construction}
\label{subsec:graph}
\vspace{-2mm}
\paragraph{Node Set $V$.}
Traditional lexicons, like General Inquirer~\cite{stone66}, usually consist of polarized unigrams. %that can be widely applied in different domains or genres of data. 
As we mentioned in Section~\ref{sec:intro}, unigrams lack the capability of capturing the sentiment conveyed in online discussions. Instead, bigrams, dependency relations, and even punctuation can serve as supplement to the unigrams. Therefore, we consider four types of \textit{text units} as nodes in the graph: unigrams, bigrams, dependency relations, sentiment dependency relations. Sentiment dependency relations are described in Section~\ref{sub:sentimentfeatures}. We replace all relation names with a general label.
%the subset of dependency relations that contains opinion words. We replace the opinion words with their polarity equivalents. For example, relation ``nsubj(wrong, you)" is in the form of ``nsubj(\texttt{SentiWord}$_{neg}$, you)". 
%Since the space of all possible text units is huge and noisy in online data, 
Text units that appear in at least 10 discussions are retained as nodes to reduce noise.
%Since the space of all possible text units is huge and noisy in online data, we only retain text units that appear in at least 10 discussions as nodes.
\vspace{-2mm}
\paragraph{Edge Set $E$.}
%As \newcite{Velikovich:2010:VWP:1857999.1858118} and \newcite{conf/acl/FengKKC13} notice, if we construct a complete graph and assign edge weights with text similarity scores, the graph is susceptible to propagating noise, and will not scale well over large number of nodes. 
As \newcite{Velikovich2010VWP} and \newcite{conf/acl/FengKKC13} notice, a dense graph with a large number of nodes is susceptible to propagating noise, and will not scale well. We thus adopt the algorithm in \newcite{conf/acl/FengKKC13} to construct a sparsely connected graph. For each text unit $t$, we first compute its representation vector $\vec a$ using Pairwise Mutual Information scores with respect to the top 50 co-occuring text units. We define ``co-occur" as text units appearing in the same sentence. An edge is created between two text units $t_{0}$ and $t_{1}$ only if they ever co-occur. The similarity between $t_{0}$ and $t_{1}$ is calculated as the Cosine similarity between $\vec a_{0}$ and $\vec a_{1}$. 

\vspace{-2mm}
\paragraph{Seed Words.}
The seed sentiment are collected from three existing lexicons: MPQA lexicon, General Inquirer, and SentiWordNet. Each word in SentiWordNet is associated with a positive score and a negative score; words with a polarity score larger than 0.7 are retained. We remove words with conflicting sentiments.

%The seed sentiment words are collected from three existing lexicons: MPQA lexicon~\cite{Wilson:2005:RCP:1220575.1220619}, General Inquirer~\cite{stone66}, and SentiWordNet~\cite{Esuli2006sentiwordnet}. Each word in SentiWordNet is associated with a positive score and a negative score, words with a polarity score larger than 0.7 are retained for use. We remove words with conflicting sentiments from different lexicons.
\vspace{-2mm}
\subsection{Data}
\vspace{-2mm}
The graph is constructed based on Wikipedia talk pages. We download the 2013-03-04 Wikipedia data dump, which contains 4,412,582 talk pages. Since we are interested in conversational languages, we filter out talk pages with fewer than 5 participants. This results in a dataset of 20,884 talk pages, from which the graph is constructed.%We use Standford parser~\cite{stanford_dependencies} to obtain dependency relations.



==> sentiment.tex <==
\begin{table*}[ht]
\centering
    {\fontsize{8}{9}\selectfont
	\begin{tabular}{|l|ccc|ccc|}
    \hline
	&\multicolumn{3}{|c|}{\textbf{Strict F1}}&\multicolumn{3}{|c|}{\textbf{Soft F1}}\\\hline
	& \textbf{Agree} & \textbf{Disagree} & \textbf{Neutral} & \textbf{Agree} & \textbf{Disagree} & \textbf{Neutral} \\ \hline
	Baseline (Polarity) & 14.56 & 25.70 & 64.04 & 22.53 & 38.61 & 66.45\\ 
	Baseline (Distance) & 8.08 & 20.68 & 84.87 & 33.75 & 55.79 & 88.97 \\ \hline
	SVM (3-way) & 26.76& 35.79& 77.39& 44.62 & 52.56 & 80.84\\ 
	~~~~ + downsampling & ~~~~ 21.60 & ~~~~ 36.32 & ~~~~ 72.11 & ~~~~ 31.86 & ~~~~ 49.58 & ~~~~ 74.92\\ 
	CRF (3-way) & 20.99& 23.85& 85.28 & 56.28 & 56.37& 89.41\\ 
	CRF (5-way) & 20.47& 19.42& 85.86 & 58.39& 56.30 & 90.10\\ 
	~~~~ + downsampling & ~~~~ 24.26& ~~~~ 31.28& ~~~~ 77.12& ~~~~ 47.30& ~~~~ 46.24& ~~~~ 80.18\\ \hline
	isotonic CRF & 24.32& 21.95& 86.26& 60.06& 58.31 & 90.51\\ 
	~~~~ + downsampling & ~~~~ 29.62& ~~~~ 34.17& ~~~~ 80.97 & ~~~~ 55.38 & ~~~~ 53.00 & ~~~~ 84.56\\ 
	~~~~ + new lexicon & \textbf{46.01} & \textbf{\textit{51.49}} & \textit{87.40} & \textbf{\textit{74.47}} & \textbf{\textit{67.02}} & \textit{90.56}\\ 
	~~~~ + new lexicon + downsampling& ~~~~ \textbf{\textit{47.90}} & ~~~~ \textbf{49.61} & ~~~~ 81.60& ~~~~ 64.97& ~~~~ 58.97 & ~~~~ 84.04\\ \hline

	\end{tabular}
	}
	\vspace{-4mm}
    \caption{\small Strict and soft F1 scores for agreement and disagreement detection on Wikipedia talk pages (AAWD). In each column, \textbf{bold} entries (if any) are statistically significantly higher than all the rest, and the \textit{italic} entry has the highest absolute value.
    %Numbers in \textbf{bold} are statistically significantly higher than the results by all the other systems above it (paired-$t$ test, $p<0.05$). Numbers in \textit{italics} represents the best results in the corresponding column. 
    Our model based on the isotonic CRF with the new lexicon produces significantly better results than all the other systems for agreement and disagreement detection. Downsampling, however, is not always helpful.}
	\label{tab:aawd_main}
\end{table*}




In this section, we test our sentiment prediction model on identifying agreement and disagreement in two types of online discussions -- \textit{Wikipedia talk pages} and \textit{online debates}.
This tagging model will be used to detect disputes from online discussions, as elaborated in the next section.
\vspace{-2mm}
\subsection{Experimental Setup}
\vspace{-2mm}
\paragraph{Datasets.}
The first dataset we use is \textit{Authority and Alignment in Wikipedia Discussions (AAWD)} corpus~\cite{Bender:2011:ASA}.
AAWD consists of 221 English Wikipedia discussions with agreement and disagreement annotations.\footnote{\scriptsize \newcite{Bender:2011:ASA} originally use positive alignment and negative alignment to indicate two types of social moves. They define those alignment moves as ``agreeing or disagreeing" with the target. We thus use agreement and disagreement instead of positive and negative alignment in this work.} %The average turn number is 15.77 for each discussion.

The annotation of AAWD is made at utterance- or turn-level, where a turn is defined as continuous body of text uttered by the same participant. Annotators either label each utterance as agreement, disagreement or neutral, and select the corresponding spans of text, or label the full turn. Each turn is annotated by two or three people. To induce an utterance-level label for instances that have only a turn-level label, we assume they have the same label as the turn.

To train our sentiment model, we further transform agreement and disagreement labels into the five sentiment labels. For utterances that are annotated as agreement and have the text span specified by at least two annotators, they are treated as very positive (PP). If an utterance is only selected as agreement by one annotator or it gets the label by turn-level annotation, it is positive (P). Very negative (NN) and negative (N) are collected in the same way from disagreement label. All others are neutral (O).
In total, we have 16,501 utterances. 1,930 and 1,102 utterances are labeled as ``NN" and ``N". 532 and 99 of them are ``PP" and ``P". All other 12,648 are neutral samples.~\footnote{\scriptsize 345 samples with both positive and negative labels are treated as neutral.}

The second dataset is the \textit{Internet Argument Corpus (IAC)}~\cite{WALKER12} collected from an online debate forum. Each discussion in IAC consists of multiple posts, where we treat each post as a turn. Most posts (72.3\%) contain quoted content from the posts they target at or other resources. A post can have more than one quote, which naturally break the post into multiple segments. 1,806 discussions are annotated with agreement and disagreement on the segment-level from -5 to 5, with -5 as strongly disagree and 5 as strongly agree.
%There are 111,569 posts in the 1806 discussions, and each post consists of multiple segments, where each segment is a response to a certain previous post. 7090 posts are annotated on segment level. 
We first compute the average score for each segment among different annotators and transform the score into sentiment label in the following way. We treat $[-5, -3]$ as NN (1595 segments), $(-3, -1]$ as N (4548 segments), $[1, 3)$ as P (911 samples), $[3, 5]$ as PP (199), all others as O (290 segments). 
%Among those annotated segments, 1,973 of them are agreement, 7,717 are disagreement, and 290 are neutral.

In the test phase, utterances or segments predicted with NN or N are treated as disagreement; the ones predicted as PP or P are agreement; O is neutral.

%\paragraph{Lexicon}
% We use the three lexicons along with our online discussion lexicon induced in Section~\ref{sec:lexicon}. Again, we remove the words if there is conflicting polarity with them. 
\vspace{-2mm}
\paragraph{Comparison.}
We compare with two baselines. (1) Baseline (Polarity) is based on counting the sentiment words from our lexicon. An utterance or segment is predicted as agreement if it contains more positive words than negative words, or disagreement if more negative words are observed. Otherwise, it is neutral. (2) Baseline (Distance) is adopted from~\cite{Hassan:2010:WAI:1870658.1870779}. Each sentiment word is associated with the closest second person pronoun, and a surface distance can be computed between them. A classifier based on Support Vector Machines~\cite{Joachims:1999:MLS:299094.299104} (SVM) is trained with the features of minimum, maximum, and average of the distances.

We also compare with two state-of-the-art methods that are widely used in sentiment prediction for conversations. The first one is an RBF kernel SVM based approach,  which has been used for sentiment prediction~\cite{Hassan:2010:WAI:1870658.1870779}, and (dis)agreement detection~\cite{Yin:2012:ULG:2392963.2392978} in online debates.
The second is CRF, which has been utilized for (dis)agreement identification in broadcast conversations~\cite{Wang:2011:DAD}.


\vspace{-2mm}
\subsection{Agreement and Disagreement Prediction}

%\begin{table*}[ht]
%\centering
%    {\small
%	\begin{tabular}{|l|ccc|ccc|}
%    \hline
%	&\multicolumn{3}{|c|}{\textbf{Strict F1}}&\multicolumn{3}{|c|}{\textbf{Soft F1}}\\\hline
%	& \textbf{Agree} & \textbf{Disagree} & \textbf{Neutral} & \textbf{Agree} & \textbf{Disagree} & \textbf{Neutral} \\ \hline
%	Baseline (Polarity) & 14.56 & 25.70 & 64.04 & 22.53 & 38.61 & 66.45\\ 
%	Baseline (Distance) & 8.08 & 20.68 & 84.87 & 33.75 & 55.79 & 88.97 \\ \hline
%	SVM (3-way) & 26.76& 35.79& 77.39& 44.62 & 52.56 & 80.84\\ 
%	~~~~ + downsampling & ~~~~ 21.60 & ~~~~ 36.32 & ~~~~ 72.11 & ~~~~ 31.86 & ~~~~ 49.58 & ~~~~ 74.92\\ 
%	CRF (3-way) & 20.99& 23.85& 85.28 & 56.28 & 56.37& 89.41\\ 
%	CRF (5-way) & 20.47& 19.42& 85.86 & 58.39& 56.30 & 90.10\\ 
%	~~~~ + downsampling & ~~~~ 24.26& ~~~~ 31.28& ~~~~ 77.12& ~~~~ 47.30& ~~~~ 46.24& ~~~~ 80.18\\ \hline
%	isotonic CRF & 24.32& 21.95& 86.26& 60.06& 58.31 & 90.51\\ 
%	~~~~ + downsampling & ~~~~ 29.62& ~~~~ 34.17& ~~~~ 80.97 & ~~~~ 55.38 & ~~~~ 53.00 & ~~~~ 84.56\\ 
%	~~~~ + new lexicon & \textbf{46.01} & \textbf{\textit{51.49}} & \textit{87.40} & \textbf{\textit{74.47}} & \textbf{\textit{67.02}} & \textit{90.56}\\ 
%	~~~~ + new lexicon + downsampling& ~~~~ \textbf{\textit{47.90}} & ~~~~ \textbf{49.61} & ~~~~ 81.60& ~~~~ 64.97& ~~~~ 58.97 & ~~~~ 84.04\\ \hline
%
%	\end{tabular}
%	}
%	\vspace{-4mm}
%    \caption{\small Strict and soft F1 scores for agreement and disagreement detection on Wikipedia talk pages (AAWD). In each column, \textbf{bold} entries (if any) are statistically significantly higher than all the rest, and the \textit{italic} entry has the highest absolute value.
%    %Numbers in \textbf{bold} are statistically significantly higher than the results by all the other systems above it (paired-$t$ test, $p<0.05$). Numbers in \textit{italics} represents the best results in the corresponding column. 
%    Our model based on the isotonic CRF with the new lexicon produces significantly better results than all the other systems for agreement and disagreement detection. Downsampling, however, is not always helpful.}
%	\label{tab:aawd_main}
%\end{table*}
%
%
%\begin{table}[ht]
%\hspace{-3mm}
%    {\small
%	\begin{tabular}{|l|ccc|}
%    \hline
%	&\textbf{Agree} & \textbf{Disagree} & \textbf{Neu}\\ \hline
%	Baseline (Polarity) & 3.33& 5.96 & 65.61\\ 
%	Baseline (Distance) & 1.65 & 5.07 & 85.41\\ \hline
%	SVM (3-way) & 25.62& 69.10 & 31.47\\ 
%	~~~~ + new lexicon features & ~~~~ 28.35& ~~~~ 72.58& ~~~~ 34.53\\ 
%	CRF (3-way) & 29.46& 74.81& 31.93\\ 
%	CRF (5-way) & 24.54& 69.31& 39.60\\ 
%	~~~~ + new lexicon features & ~~~~ 28.85& ~~~~ 71.81& ~~~~ 39.14\\ \hline
%	isotonic CRF & \textbf{53.40} & \textbf{76.77}& \textit{44.10}\\ 
%	~~~~ + new lexicon  & ~~~~ \textbf{\textit{61.49}} & ~~~~ \textbf{\textit{77.80}}& ~~~~ \textit{51.43}\\ \hline
%
%	\end{tabular}
%	}
%	\vspace{-4mm}
%    \caption{\small F1 scores for agreement and disagreement detection on online debate (IAC). In each column, \textbf{bold} entries (if any) are statistically significantly higher than all the rest, and the \textit{italic} entry has the highest absolute value except baselines.
%    %Numbers in \textbf{bold} are statistically significantly higher than the results by all the other systems above it (paired-$t$ test, $p<0.05$). Numbers in \textit{italics} are significantly better than SVM and CRF based approaches. 
%    We have two main observations: 1) Both of our models based on isotonic CRF significantly outperform other systems for agreement and disagreement detection. 2) By adding the new lexicon, either as features or constraints in isotonic CRF, all systems achieve better F1 scores.}
%    \label{tab:iac_main}
%
%\end{table}

% We test our model on the discussions from Wikipedia talk page (AAWD) and online debate (IAC). Since we hypothesize that sentiment analysis alone can be employed for agreement and disagreement detection, we use the following schema to get agreement and disagreement categories. Utterances or segments labeled with NN or N are treated as disagreement, utterances predicted as PP or P are agreement, and O is neutral.

We evaluate the systems by standard F1 score on each of the three categories: agreement, disagreement, and neutral. For AAWD, we compute two versions of F1 scores. \textbf{Strict F1} is computed against the true labels. For \textbf{soft F1}, if an utterance is never labeled by any annotator on the utterance-level and adopts its agreement/disagreement label from the turn-level annotation, then it is treated as a true positive when predicted as neutral. 

\begin{table}[ht]
%\hspace{-3mm}
    {\fontsize{8}{9}\selectfont
	\begin{tabular}{|l|ccc|}
    \hline
	&\textbf{Agree} & \textbf{Disagree} & \textbf{Neu}\\ \hline
	Baseline (Polarity) & 3.33& 5.96 & 65.61\\ 
	Baseline (Distance) & 1.65 & 5.07 & 85.41\\ \hline
	SVM (3-way) & 25.62& 69.10 & 31.47\\ 
	~~~~ + new lexicon features & ~~~~ 28.35& ~~~~ 72.58& ~~~~ 34.53\\ 
	CRF (3-way) & 29.46& 74.81& 31.93\\ 
	CRF (5-way) & 24.54& 69.31& 39.60\\ 
	~~~~ + new lexicon features & ~~~~ 28.85& ~~~~ 71.81& ~~~~ 39.14\\ \hline
	isotonic CRF & \textbf{53.40} & \textbf{76.77}& \textit{44.10}\\ 
	~~~~ + new lexicon  & ~~~~ \textbf{\textit{61.49}} & ~~~~ \textbf{\textit{77.80}}& ~~~~ \textit{51.43}\\ \hline

	\end{tabular}
	}
	\vspace{-4mm}
    \caption{\small F1 scores for agreement and disagreement detection on online debate (IAC). In each column, \textbf{bold} entries (if any) are statistically significantly higher than all the rest, and the \textit{italic} entry has the highest absolute value except baselines.
    %Numbers in \textbf{bold} are statistically significantly higher than the results by all the other systems above it (paired-$t$ test, $p<0.05$). Numbers in \textit{italics} are significantly better than SVM and CRF based approaches. 
    We have two main observations: 1) Both of our models based on isotonic CRF significantly outperform other systems for agreement and disagreement detection. 2) By adding the new lexicon, either as features or constraints in isotonic CRF, all systems achieve better F1 scores.}
    \label{tab:iac_main}

\end{table}

Table~\ref{tab:aawd_main} demonstrates our main results on the AAWD dataset. Without downsampling, our isotonic CRF based systems with the new lexicon significantly outperform the compared approaches for agreement and disagreement detection according to the paired-$t$ test ($p<0.05$). We also perform downsampling by removing the turns with all neutral utterances. However, it does not always help with performance.

Similarly, the results on the IAC dataset are displayed in Table~\ref{tab:iac_main}. Both of our systems based on isotonic CRF achieve significantly better F1 scores than the comparison. Especially, our system with the new lexicon produces the best results. For SVM and CRF based systems, we also add new sentiment features constructed from the new lexicon as described in Section~\ref{sub:sentimentfeatures}. We can see that those sentiment features also boost the performance for SVM and CRF based classifiers. To compare with the state-of-the-art system~\cite{Abbott:2011:YST} on IAC, we also build a balanced dataset consisting of agreement and disagreement as~\newcite{Abbott:2011:YST} do. We achieve an accuracy of 0.64, which is comparable to 0.68 reported by~\newcite{Abbott:2011:YST}.

\vspace{-2mm}
\paragraph{Feature Evaluation.}
We evaluate the effectiveness of features by adding one type of features each time. The results can be found in Table~\ref{tab:aawd_diff_featureset}.% and Table~\ref{tab:iac_diff_featureset}.

In addition, we utilize $\chi^{2}$-test to highlight some of the salient features on the two datasets. We can see from Table~\ref{tab:feature_analysis} that, for online debates (IAC), some features are highly topic related, such as ``\textit{the male}" or ``\textit{the scientist}". This observation concurs with the conclusion in~\newcite{misra-walker:2013:SIGDIAL} that features with topic information are indicative for agreement and disagreement detection.


\begin{table}[ht]

    {\fontsize{8}{9}\selectfont
%    \hspace{-3mm}
	\begin{tabular}{|l|ccc|}
    \hline

	\textbf{AAWD} & \textbf{Agree} & \textbf{Disagree} & \textbf{Neu}\\ \hline
	Lex & 40.77 & 52.90 & 79.65\\ \hline
	Lex + Syn & 68.18 & 63.91 & 88.87 \\ \hline
	Lex + Syn + Disc  & 70.93 & 63.69& 89.32\\ \hline
	Lex + Syn + Disc + Con  &  71.27& 63.72 &  89.60\\ \hline
	Lex + Syn + Disc + Con + Sent  & \textbf{74.47} & \textbf{67.02} & 90.56\\ \hline
	\end{tabular}
	}

	{\fontsize{8}{9}\selectfont
%	\hspace{-3mm}
	\begin{tabular}{|l|ccc|}
    \hline
	\textbf{IAC} &\textbf{Agree} & \textbf{Disagree} & \textbf{Neu}\\ \hline
	Lex & 56.65& 75.35& 45.72\\ \hline
	Lex + Syn & 54.16& 75.13& 46.12\\ \hline
	Lex + Syn + Disc & 54.27& 76.41& 47.60\\ \hline
	Lex + Syn + Disc + Con & 55.31& 77.25& 48.87\\ \hline
	Lex + Syn + Disc + Con + Sent  & \textbf{61.49} & 77.80 & \textbf{51.43}\\ \hline
	\end{tabular}
	}
	\vspace{-4mm}
    \caption{\small Results on Wikipedia talk page (AAWD) (with soft F1 score) and online debate (IAC) with different feature sets (i.e \textbf{Lex}ical, \textbf{Syn}tacitc/Semantic, \textbf{Disc}ourse, \textbf{Con}versation, and \textbf{Sent}iment features) by using isotonic CRF. The numbers in \textbf{bold} are statistically significantly higher than the numbers above it (paired-$t$ test, $p<0.05$).}
    \label{tab:aawd_diff_featureset}

\end{table}



%\begin{table}[ht]
%\centering
%    {\small
%	\begin{tabular}{|l|ccc|}
%    \hline
%	&\textbf{Agree} & \textbf{Disagree} & \textbf{Neu}\\ \hline
%	Lex & 56.65& 75.35& 45.72\\ \hline
%	Lex + Syn & 54.16& 75.13& 46.12\\ \hline
%	Lex + Syn + Disc & 54.27& 76.41& 47.60\\ \hline
%	Lex + Syn + Disc + Con & 55.31& 77.25& 48.87\\ \hline
%	Lex + Syn + Disc + Con + Sent  & \textbf{61.49} & 77.80 & \textbf{51.43}\\ \hline
%	\end{tabular}
%	}
%	\vspace{-4mm}
%    \caption{\small Results on online debate (IAC) with different feature sets by using isotonic CRF. The numbers in \textbf{bold} are statistically significantly higher than the numbers above it (paired-$t$ test, $p<0.05$).}
%    \label{tab:iac_diff_featureset}
%
%\end{table}



\begin{table}[ht]

    {\fontsize{8}{9}\selectfont
    \begin{tabular}{|p{72mm}|}
    \hline
    \textbf{AAWD} \\
	\underline{\textsc{Positive}}:
	agree, nsubj (agree, I), nsubj (right, you), Rel (Sentiment$_{pos}$, I), thanks, amod (idea, good), nsubj(glad, I), good point, concur, happy with, advmod (good, pretty), suggestion$_{Hedge}$\\ 
	
	\underline{\textsc{Negative}}: 
	you, your, nsubj (negative, you), numberOfNegator, don't, nsubj (disagree, I), actually$_{SentInitial}$, please stop$_{SentInitial}$, what ?$_{SentInitial}$, should$_{Hedge}$\\ \hline
	\end{tabular}
	}
	
	{\fontsize{8}{9}\selectfont
	\begin{tabular}{|p{72mm}|}
    \hline
    \textbf{IAC} \\
	\underline{\textsc{Positive}}:
	amod (conclusion, logical), Rel (agree, on), Rel (have, justified), Rel (work, out), one might$_{SentInitial}$, to confirm$_{Hedge}$, women\\
	
	\underline{\textsc{Negative}}:
	their kind, the male, the female, the scientist, according to, is stated, poss (understanding, my), hell$_{SentInitial}$, whatever$_{SentInitial}$\\ \hline
	\end{tabular}
	}
	\vspace{-4mm}
    \caption{\small Relevant features by $\chi^{2}$ test on AAWD and IAC.}
    \label{tab:feature_analysis}

\end{table}





%\begin{table}[ht]
%\centering
%    {\small
%	\begin{tabular}{|p{72mm}|}
%    \hline
%	\textsc{Positive}\\ \hline
%	amod (conclusion, logical), Rel (agree, on), Rel (have, justified), Rel (work, out), one might$_{SentInitial}$, to confirm$_{Hedge}$, women\\ \hline
%	\textsc{Negative} \\ \hline
%	their kind, the male, the female, the scientist, according to, is stated, poss (understanding, my), hell$_{SentInitial}$, whatever$_{SentInitial}$\\ \hline
%	\end{tabular}
%	}
%    \caption{Feature analysis by using $\chi^{2}$ test.}
%    \label{tab:iac_feature_analysis}
%
%\end{table}

